Detection and Measurement of Syntactic Templates in Generated Text

Recent work on evaluating the diversity of text generated by LLMs has focused on word-level features. Here we offer an analysis of syntactic features to characterize general repetition in models, beyond frequent n-grams. Specifically, we define syntactic templates and show that models tend to produce templated text in downstream tasks at a higher rate than what is found in human-reference texts. We find that most (76%) templates in model-generated text can be found in pre-training data (compared to only 35% of human-authored text), and are not overwritten during fine-tuning processes such as RLHF. This connection to the pre-training data allows us to analyze syntactic templates in models where we do not have the pre-training data. We also find that templates as features are able to differentiate between models, tasks, and domains, and are useful for qualitatively evaluating common model constructions. Finally, we demonstrate the use of templates as a useful tool for analyzing style memorization of training data in LLMs.

==> figures/ex_templates.tex <==
\begin{figure}
    \centering
    \resizebox{0.5\textwidth}{!}{\includegraphics[width=0.5\linewidth]{figures/img/ex_templates_small.pdf}
    }
    \caption{Example templates from the Rotten Tomatoes dataset and their frequency. Some templates are shared between human-written references and model-generated summaries. \ye{was this being referred somewhere?}}
    \label{fig:template_themes}
\end{figure}

==> figures/percent_templates.tex <==
\begin{figure}
    \centering
    \resizebox{0.5\textwidth}{!}{
    \includegraphics{figures/img/percent_templates.pdf}
    }
    \caption{Percentage of outputs with $\geq$1 template of size $n = 6$ as (a) top p and (b) temperature increase. Templates still appear in over 80\% of outputs, even in degenerative cases (as temperature approaches 2).}
    \label{fig:percent_templates}
\end{figure}

==> figures/pretraining_data_overlap.tex <==
\begin{figure}
    \centering
\resizebox{0.48\textwidth}{!}{    \includegraphics{figures/img/template_coverage_training_data.pdf}
}
    \caption{\todo{add ci} Coverage of templates found in (a) pre-training data, (b) fine-tuning data, and (c) both datasets combined. Templates are found at a much higher rate in the training data than random n-gram sequences.}
    \label{fig:coverage}
\end{figure}

==> figures/temperature_llama_olmo.tex <==
\begin{figure}
    \centering
    \resizebox{0.49\textwidth}{!}{
    \includegraphics{figures/img/temperature.pdf}
    }
    \caption{Diversity, length, and evaluation metrics shown as \texttt{Temperature} is increased during sampling. Compression ratios (CR) for both tokens and POS decrease indicating an \textit{increase} in diversity. Similarly, N-Gram Diversity shows an increase in diversity. ROUGE-1 scores and average summary length stay relatively stable, while bigram overlap with the input slightly increases.}
    \label{fig:cr_temperature}
\end{figure}

==> figures/top_p_llama_olmo.tex <==
\begin{figure}
    \centering
    \resizebox{0.5\textwidth}{!}{
    \includegraphics{figures/img/top_p.pdf}
    }
    \caption{Diversity, length, and evaluation metrics shown as \texttt{Top P} is increased during sampling. Compression ratios (CR) for both tokens and POS decrease indicating an \textit{increase} in diversity. Similarly, N-Gram Diversity shows an increase in diversity. ROUGE-1 scores and average summary length stay relatively stable, while bigram overlap with the input slightly increases.}
    \label{fig:cr_top_p}
\end{figure}

==> tables/cr_pos_booookscore_increm.tex <==
\begin{table}
\begin{centering}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lrr}
  &  \multicolumn{2}{c}{\textbf{BooookScore, Incremental}}\\
\toprule
 \textbf{Model}&  \textbf{\begin{tabular}[r]{@{}r@{}} CR: \\POS\end{tabular}}& \textbf{\textbf{\begin{tabular}[r]{@{}r@{}}$\geq1$ Templates\\\% ($n=6$)\end{tabular}}}    \\ \midrule
  % \emoji{robot}\ \ \ 
  
  Claude-2048&  5.71& 86.0 (0.007)\\
 Claude-88000&  5.60& 96.0 (0.010)\\
 ChatGPT-2048&  5.76& 95.0 (0.011)\\
 GPT4-2048&  5.95& 99.0 (0.009)\\
 GPT4-4096&  6.05& 100.0 (0.010)\\

  Mixtral-2048&  5.59& 99.0 (0.012)\\\bottomrule
\end{tabular}
}
\caption{Compression ratio with POS (CR-POS) reported for  the BooookScore dataset. We report the percentage of generated outputs with at least 1 template of size $n=6$, and the rate of templates-per-token in parentheses.}
\label{tab:cr_pos_booookscore_incr}
\end{centering}

\end{table}


==> tables/cr_pos_dolma_100.tex <==
\begin{table}
\begin{centering}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{llll}
\toprule
 \textbf{Model}& \textbf{\begin{tabular}[c]{@{}l@{}} CR: \\POS\end{tabular}}&\textbf{\begin{tabular}[c]{@{}l@{}} Avg. Text \\Length\end{tabular}}&\textbf{\textbf{\begin{tabular}[c]{@{}l@{}}$\geq1$ Templates\\\% ($n=6$)\end{tabular}}}   \\ \midrule
  % \emoji{robot}\ \ \ 
  
  OLMo-7B     & 5.648&483.193&82.6 (0.012)\\\bottomrule
\end{tabular}
}
\caption{\note{appendix?} Compression ratio with POS (CR-POS) reported for  the a sampled subset of Dolma. We report the percentage of generated outputs with at least 1 template of size $n=6$, and the rate of templates-per-token in parentheses (avg. num. templates per summary normalized by avg. length) for OLMo.}
\label{tab:cr_pos_dolma_100}
\end{centering}

\end{table}


==> tables/overlap_prompt.tex <==
\begin{table}[]
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lll}
\toprule
 \textbf{Prompt}&  \textbf{Input Docs (\%)}& \textbf{Refs (\%)}\\ \midrule
 Please write a summary.                                                                                  &  34.2& 27.4\\
 \begin{tabular}[c]{@{}l@{}}Please write a summary \\ \ \ of the movie reviews.\end{tabular}                  &  36& 27.4\\
 Summarize.                                                                                               &  35.6& 29.2\\
 Write a short summary.                                                                                   &  34.8& 28.6\\
  \begin{tabular}[c]{@{}l@{}}Write a short summary \\ \ \ and be creative.\end{tabular}                        & 37.8& 31.6\\

 Write a meta-analysis.                                                                                   & 36.8& 27\\
 \begin{tabular}[c]{@{}l@{}}Write an aggregate movie \\ \ \ review based on the\\  \ \ above reviews.\end{tabular} & 35.4& 29.4\\
   \midrule
\end{tabular}
}
\caption{Overlap percentage of templates between OLMo and (a) the input documents and (b)  references across different templates.}
\label{tab:overlap_percentages}
\end{table}


==> tables/regression.tex <==
\begin{table}[]
\centering
\resizebox{0.5 \textwidth}{!}{
\begin{tabular}{lllll}
\toprule
 \textbf{Model}&  \textbf{Words}& \textbf{Templates}&  \textbf{\begin{tabular}[l]{@{}l@{}} BOW +\\Templates \end{tabular}}&\textbf{POS}\\ \midrule
 Alpaca-7B&  0.91& 0.86&                   0.92&0.81\\
 Llama-2-7B&  0.81& 0.78&                   0.87&0.66\\
 Mistral-7B&  0.90& 0.86&                   0.97&0.75\\
 OLMo-7B&  0.82& 0.81&                   0.88&0.65\\
\midrule
  Macro Avg.& 0.86& 0.83&  0.91&0.71\\
  \midrule
\end{tabular}
}
\caption{F1 scores reported for multinomial regression with Bag-of-Words, -Templates, and -Part-of-Speech features (POS) on the Rotten Tomatoes dataset.}
\label{tab:logistic_regression}
\end{table}




==> tables/regression_avg.tex <==
\begin{table}[]
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{llll}
\toprule
 \textbf{Prompt}&  \textbf{Words}& \textbf{Templates}& \textbf{POS}\\ \midrule
 Please write a summary.                                                                                  &  0.86& 0.83&                  0.71\\
 \begin{tabular}[c]{@{}l@{}}Please write a summary \\ \ \ of the movie reviews.\end{tabular}                  &  0.87& 0.86&                  0.80\\
 Summarize.                                                                                               &  0.78& 0.78&                  0.65\\
 Write a short summary.                                                                                   &  0.80& 0.79&                  0.67\\
  \begin{tabular}[c]{@{}l@{}}Write a short summary \\ \ \ and be creative.\end{tabular}                        & 0.91& 0.90& 0.81\\

 Write a meta-analysis.                                                                                   & 0.90& 0.90&0.79\\
 \begin{tabular}[c]{@{}l@{}}Write an aggregate movie \\ \ \ review based on the\\  \ \ above reviews.\end{tabular} & 0.90& 0.87&0.80\\
   \midrule
\end{tabular}
}
\caption{Multinomial regression with Bag-of-Words, -Templates, and -Part-of-Speech (POS) features on the Rotten Tomatoes dataset. \textbf{Macro average} \textbf{F1} is reported for the one-vs-all model identification task across all prompts. Classification performance varies between prompts.}
\label{tab:logistic_regression_all_prompts}
\end{table}

